Second-order group knockoffs with applications to GWAS

Conditional testing via the knockoff framework allows one to identify -- among large number of possible explanatory variables -- those that carry unique information about an outcome of interest, and also provides a false discovery rate guarantee on the selection. This approach is particularly well suited to the analysis of genome wide association studies (GWAS), which have the goal of identifying genetic variants which influence traits of medical relevance. While conditional testing can be both more powerful and precise than traditional GWAS analysis methods, its vanilla implementation encounters a difficulty common to all multivariate analysis methods: it is challenging to distinguish among multiple, highly correlated regressors. This impasse can be overcome by shifting the object of inference from single variables to groups of correlated variables. To achieve this, it is necessary to construct "group knockoffs." While successful examples are already documented in the literature, this paper substantially expands the set of algorithms and software for group knockoffs. We focus in particular on second-order knockoffs, for which we describe correlation matrix approximations that are appropriate for GWAS data and that result in considerable computational savings. We illustrate the effectiveness of the proposed methods with simulations and with the analysis of albuminuria data from the UK Biobank. The described algorithms are implemented in an open-source Julia package Knockoffs.jl, for which both R and Python wrappers are available.

==> Algo.tex <==
Though the construction of Gaussian group knockoffs reduces to choosing the matrix $\bS$ in Equation \eqref{G_S} or \eqref{eq:G_Smult}, the problem of how to do so presents unsolved computational issues. \cite{dai2016knockoff} considers the SDP objective and opt to take $\bS_i = \gamma \bSigma_{G_i, G_i}$ for some shared scalar $\gamma$. This conveniently reduces the optimization to a one-dimensional problem. However, in doing so, it fails to reap the full benefit of the relaxed group knockoffs conditions, in which $\bS$ has substantially more free parameters. As a result, we find that it often exhibits low power. 

We thus consider two alternatives of varying computational complexity, both aiming to obtain a greater share of these benefits. In the first, which we call full optimization, we optimize over every entry of $\bS$. This can be a substantial number of variables, so we also consider an alternative, which we call PCA optimization. In the latter approach, we restrict $\bS$ to be a linear combination of the eigenvectors of 
$$\bSigma_{blocked} = \begin{bmatrix} \bSigma_1 & & \\ & \ddots & \\ & & \bSigma_G \end{bmatrix}.$$
This interpolates between the one-dimensional optimization of \cite{dai2016knockoff} and the full optimization. Because of the block diagonal structure of $\bSigma_{blocked}$, its eigenvectors can be computed very efficiently. In practice, we have success alternating between full and PCA optimization. 

In each case, we solve for $\bS$ via a simple algorithm that we call coordinate descent. Our approach is inspired by recent work in this area \citep{spector2022powerful, askari2021fanok}. In the PCA optimization, this involves precomputing the eigenvectors $(\bv_1,..., \bv_p)$ of $\bSigma_{blocked}$ and successively performing rank-1 updates
$$\bS^{new} = \bS + \delta \bv_i \bv_i^t$$
This breaks the problem into a sequence of one-dimensional optimizations over $\delta$. The exact form of $\delta$ varies for different objectives, but in the case of ME knockoffs, we can explicitly compute
\begin{eqnarray*}
    \delta &=& \frac{M\bv^t\bS^{-1}\bv - \bv^t\bD^{-1}\bv}{(M+1)\bv^t\bS^{-1}\bv\bv^t\bD^{-1}\bv}
\end{eqnarray*}
with $\bD = \frac{M+1}{M}\bSigma - \bS$. Constants such as $\bv^t\bS^{-1}\bv$ and $\bv^t\bD^{-1}\bv$ can be extracted efficiently by maintaining Cholesky factors of $\bS$ and $\bD$. Because each Cholesky update scales as $\mathcal{O}(p^2)$, group knockoffs based purely on PCA updates scales as $\mathcal{O}(p^3)$, which is equivalent to the computational complexity of regular model-X knockoffs \citep{askari2021fanok}.

Likewise, for full optimization, we successively update 
$$S_{ij}^{new} = S_{ij} + \delta.$$
In the case of ME objectives, the update to $\delta$ now requires maximizing the following problem, which is fortunately computationally efficient
\begin{eqnarray*}
    g(\delta) &=& \log\left((1 - \delta \be_i^t\bD^{-1}\be_j)^2 - \delta^2 \be_i^t\bD^{-1}\be_i\be_j^t\bD^{-1}\be_j\right) + \\
    && M\log\left((1+\delta \be_i^t\bS^{-1}\be_j)^2 - \delta^2 \be_j^t\bS^{-1}\be_j\be_i^t\bS^{-1}\be_i\right)
\end{eqnarray*}
Finally, we must ensure each update satisfies our constraints. Supplemental Section \ref{ssec:supplementccd} explains in detail how to solve these optimizations efficiently for each of SDP, MVR, and ME knockoffs and how to ensure $\bS^{new}$ satisfies each of our constraints. A summary is provided as Algorithm \eqref{alg:CCD_concise} with a more detailed version provided in the supplement as Algorithm \eqref{alg:CCD}. 



\begin{algorithm}
    \caption{Coordinate descent for group knockoffs optimization}\label{alg:CCD_concise}
    \begin{algorithmic}[1]
	\STATE { \textbf{Input:} correlation matrix $\bSigma_{p \times p}$, group membership vector, and $M$ (number of knockoffs)}
        \STATE{ \textbf{Initialize:} $\bS = \frac{1}{2}\bS_{\text{eSDP}}$ with $\bS_{\text{eSDP}}$ from  \citep{dai2016knockoff}} and $\bD = \frac{M+1}{M}\bSigma - \bS$
        \STATE{ \textbf{Compute:} ($\bv_1,...,\bv_p$) based on eigendecomposition of $\bSigma_{block}$}
        \STATE{ \textbf{Compute:} Cholesky factors $\bL\bL^t = \text{cholesky}(\bD)$ and $\bC\bC^t = \text{cholesky}(\bS)$}
	\WHILE{Not converged}
            %\STATE{\#\# PCA iterations}
            \FOR{$\bv_i \in (\bv_1,...,\bv_p)$} 
                \STATE Compute $\delta$ and perform rank-1 update: $\bS_{new} = \bS + \delta \bv_i\bv_i^t$
                \STATE Update cholesky factors $\bL_{new}\bL_{new}^t = \frac{M+1}{M}\bSigma - \bS_{new}$ and $\bC_{new}\bC_{new}^t = \bS_{new}$
		\ENDFOR
            %\STATE{\#\# Full optimization}
            \FOR{$g = \{1,...,G\}$}
                \FOR{$(i,j)$ in group $g$}
                    \STATE Compute $\delta$ and perform rank-2 update: $S^{new}_{ij} = S^{new}_{ji} = S_{ij} + \delta$
                    \STATE Update cholesky factors $\bL_{new}\bL_{new}^t = \frac{M+1}{M}\bSigma - \bS_{new}$ and $\bC_{new}\bC_{new}^t = \bS_{new}$
                \ENDFOR
            \ENDFOR
        \ENDWHILE
        \STATE \textbf{Output:} Group-block-diagonal matrix $\bS$ satisfying $\frac{M+1}{M}\bSigma - \bS \succeq 0$ and $\bS \succeq 0$.
	\end{algorithmic}
\end{algorithm}


==> Code.tex <==
We implemented the proposed algorithms in an open-sourced \texttt{Julia} \citep{bezanson2017julia} package \texttt{Knockoffs.jl} available at \url{https://github.com/biona001/Knockoffs.jl}. We also provide \texttt{R} and \texttt{Python} wrappers via the packages \texttt{knockoffsr} and \texttt{knockoffspy} available at \url{https://github.com/biona001/knockoffsr} and \url{https://github.com/biona001/knockoffspy}. To facilitate downloading and extraction of LD matrices featured in our real data analysis, we developed another software \texttt{EasyLD.jl} available at \url{https://github.com/biona001/EasyLD.jl}. Finally, scripts to reproduce our real and simulated experiments are available at \url{https://github.com/biona001/group-knockoff-reproducibility}.

==> MultipleKnockoffs.tex <==
The multiple knockoff filter was first proposed by \cite{gimenez2019improving} and used extensively in \citep{he2021genome,he2022ghostknockoff} to improve the power and stability of model-X knockoffs. 
% This method works by generating $M$ distinct knockoff copies $(\tilde{X}^1,..., \tilde{X}^M)$ that satisfy the \textit{extended exchangeability} property 
% $$(X, \tilde{X}^1,..., \tilde{X}^M)_{\text{swap}(\sigma_i)} \overset{d}{=} (X, \tilde{X}^1,..., \tilde{X}^M)$$
% for all $1 \leq i \leq p$. Here, $\sigma_i$ is any permutation of only $(X_i, \tilde{X}^1_i,..., \tilde{X}^M_i)$, leaving all other entries fixed. 
Conceptually, the benefit of using multiple knockoffs is that it removes some noise from the knockoff filter, a procedure that is random even conditional on the observed data due to the randomness of knockoff generation. 

% \subsubsection{Multiple Gaussian group knockoffs}
In the Gaussian case in which $X \sim N(\mathbf{0}, \bSigma)$, \cite{gimenez2019improving} show that $M$-group knockoffs $(X,\tilde{X}^1,..., \tilde{X}^M)$ can be generated from $N(\mathbf{0}, \bG_{\bS})$ where
\begin{eqnarray} \label{eq:G_Smult}
	\bG_{\bS} &=& 
	\begin{bmatrix}
		\bSigma & \bSigma - \bS & \cdots & \bSigma - \bS\\
		\bSigma - \bS & \bSigma & \cdots & \bSigma - \bS\\
		\vdots & \vdots & \ddots & \vdots\\
		\bSigma - \bS & \cdots & \cdots & \bSigma
	\end{bmatrix} \in \bbR^{p(M + 1) \times p(M + 1)}.
\end{eqnarray}
As in the single knockoff setting, the problem thus reduces to optimizing over $\bS$, where the constraints now translate to $0 \preceq \bS \preceq \frac{M+1}{M}\bSigma$ and $\bS = \text{diag}(\bS_1,...,\bS_G)$. We thus recover the original constraints in the case $M = 1$. Later, we derive algorithms to optimize the three objectives $L_{\text{SDP}}(\bS), L_{\text{MVR}}(\bS), L_{\text{ME}}(\bS)$ under these new constraints.

% \subsubsection{Knockoff filter to define FDR threshold $\tau$}
% Upon generating the feature importance statistics $(Z_g, \tilde{Z}_g^1,...,\tilde{Z}_g^M)$ for $X_g$ and its $M$ group knockoff copies, we define the importance score for group $g$ as
% \begin{eqnarray*}
% 	    W_g &=& \left(Z_g - \text{median}\{\tilde{Z}_g^{1},...,\tilde{Z}_g^{M}\}\right)\indic\{Z_g \ge \max\{\tilde{Z}_g^{1},...,\tilde{Z}_g^{M}\}\}.
% \end{eqnarray*}
% Let $\kappa_g = \argmax_{0\le m \le M}Z^{m}_g$ be the index of the original (denoted as $0$) or knockoff with the largest feature importance for group $g$, and let $\tau_g = Z_g^{(0)} - \text{median}\{\tilde{Z}_g^{(1)},...,\tilde{Z}_g^{(M)}\}$ where $Z_g^{(0)} \ge Z_g^{(1)} \ge ... \ge Z_g^{(M)}$ are the ordered statistic of $Z_g$ and its $M$ knockoffs. Note that $W_g \ge 0$ always, and $W_g$ is nonzero if and only if $\kappa_g = 0$, i.e., the original group has larger feature importance than all of its knockoffs. 

% With importance scores computed for each group, the data dependent threshold becomes
% \begin{eqnarray*}
%     \tau &=& \min \left\{t > 0 : \frac{\frac{1}{M} + \frac{1}{M} \# \{\kappa_g \ge 1, \tau_g \ge t\}}{\# \{\kappa_g = 0, \tau_g \ge t\}} \le q\right\},
% \end{eqnarray*}
% The procedure concludes by selecting all groups $g$ with $W_g \ge \tau$. 

%
%
%Let $T_i$ denote the importance score for variable $i$. For each group $g \in 1,...,G$, compute
%\begin{eqnarray*}
%    T_g &=& \sum_{i \in \text{ group } g} | T_i| \quad (\text{importance score of original features in group $g$})\\
%    \Tilde{T}_g^{1} &=& \sum_{i \in \text{ group } g} | \Tilde{T}_i^{1} | \quad (\text{importance score of first knockoff features in group $g$})\\
%    &\vdots&\\
%    \Tilde{T}_g^{m} &=& \sum_{i \in \text{ group } g} | \Tilde{T}_i^{m} | \quad (\text{importance score of last knockoff copy in group $g$})\\
%    \kappa_g &=& \argmax_{0\le k \le m}T^{k} \quad (\text{index of the original (denoted as 0) or knockoff feature with the largest score})\\
%    \tau_g &=& T_g^{(0)} - \text{median}_{1\le k \le m} \tilde{T}_g^{(k)} \quad (\text{largest importance score minus median of remaining scores})\\
%    W_g &=& \left[T_g - \text{median}\{\tilde{T}_g^{1},...,\tilde{T}_g^{m}\}\right]I(T_g \ge max\{\tilde{T}_g^{1},...,\tilde{T}_g^{m}\}) \quad (\text{overall importance score of group $g$})
%\end{eqnarray*}
%In multiple knockoffs, $\kappa_g$ quantifies the sign ($\kappa_g = 0$ if the original feature is more important than all its knockoffs), and $\tau_g$ quantifies the magnitude of the importance score which is invariant to swapping. The group importance scores $W_g \ge 0$ is non-zero if and only if the original feature has a larger importance score than all its knockoffs. 
%
%Once importance scores are computed for each group, define the knockoff filter threshold
%\begin{align*}
%    \tau = \min \left\{t > 0 : \frac{\frac{1}{m} + \frac{1}{m} \# \{\kappa_g \ge 1, \tau_g \ge t\}}{\# \{\kappa_g = 0, \tau_g \ge t\}} \right\}
%\end{align*}
%and groups with $W_g > \tau$ are selected. 



==> Notation.tex <==
% We suppose that we have $n$ i.i.d. samples $(X_i, Y_i)$, with $X_i \in \bbR^p$ a vector of covariates and $Y_i \in \bbR$ a response of interest. We use $\bX \in \bbR^{n \times p}$ to denote the stacked design matrix whose $i$th row is $X_i$, and we use $\bSigma$ to denote the population covariance of $X$. More generally, we use bolded uppercase text to denote matrices, bolded lowercase for vectors, and unbolded uppercase for random variables.

Let response $Y$ depend arbitrarily on covariates $X = (X_1,...,X_p)$. Given $n$ i.i.d. samples, we use $\bX \in \bbR^{n \times p}$ to denote the stacked design matrix where each row is a sample, and $\bSigma$ to denote the population covariance of $X$. Given a partition of $[p] = \{1, 2,..., p\}$ into $G$ disjoint groups of variables, we denote by $\mathcal{A}_g$ the set of variables in group $g$. 
For other variables, we will use bolded uppercase text to denote matrices, unbolded uppercase for random variables, and bolded lowercase for vectors. 
Henceforth, we assume that the groups are contiguous, as can be done without loss of generality by permuting the columns of $\bX$. 
% We use $\mathcal{C} \subseteq [G]$ to denote a subset of groups and $C = \bigcup_{g \in \mathcal{C}} \mathcal{A}_g$ to denote the variables belonging to any of these groups. 
% Similarly, we use $\bX_g$ to denote the columns of $\bX$ that are in group $g$, and we use $\bX_{-g}$ to denote all other columns.  

